Efficient Memory Partitioning in Software Defined Hardware

As programmers turn to software-defined hardware (SDH) to maintain a high level of productivity while programming hardware to run complex algorithms, heavy-lifting must be done by the compiler to automatically partition on-chip arrays. In this paper, we introduce an automatic memory partitioning system that can quickly compute more efficient partitioning schemes than prior systems. Our system employs a variety of resource-saving optimizations and an ML cost model to select the best partitioning scheme from an array of candidates. We compared our system against various state-of-the-art SDH compilers and FPGAs on a variety of benchmarks and found that our system generates solutions that, on average, consume 40.3% fewer logic resources, 78.3% fewer FFs, 54.9% fewer Block RAMs (BRAMs), and 100% fewer DSPs.

==> Makefile <==
PAPER = arxivmain
TEX = $(wildcard *.tex text/*.tex)
BIB = references.bib
FIGS = $(wildcard figs/*.pdf figs/*.png graphs/*.pdf graphs/*.png)

.PHONY: all export clean lunch

$(PAPER).pdf: $(TEX) $(BIB) $(FIGS) acmart.cls
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)

lunch: $(PAPER).pdf
	bash publish.sh $(PAPER).pdf

test: $(TEX) $(BIB) $(FIGS) acmart.cls
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)

# figs/speedupbars.tex: figs/speedupbars.gp figs/speedupbars.dat
# 	cd figs && gnuplot speedupbars.gp
# 	cd figs && sed -i.bak 's/speedupbars/figs\/speedupbars/' speedupbars.tex

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf



==> project/target/streams/$global/dependencyPositions/$global/streams/update_cache_2.12/output_dsp <==
{"{\"organization\":\"org.scala-lang\",\"name\":\"scala-library\",\"revision\":\"2.12.7\",\"configurations\":\"provided\",\"isChanging\":false,\"isTransitive\":true,\"isForce\":false,\"explicitArtifacts\":[],\"inclusions\":[],\"exclusions\":[],\"extraAttributes\":{},\"crossVersion\":{\"type\":\"Disabled\"}}":{"value":{"$fields":["path","startLine"],"path":"(sbt.Classpaths.jvmBaseSettings) Defaults.scala","startLine":2207},"type":"LinePosition"}}

==> scala/project/target/streams/_global/dependencyPositions/_global/streams/update_cache_2.12/output_dsp <==
{"{\"organization\":\"org.scala-lang\",\"name\":\"scala-library\",\"revision\":\"2.12.10\",\"configurations\":\"provided\",\"isChanging\":false,\"isTransitive\":true,\"isForce\":false,\"explicitArtifacts\":[],\"inclusions\":[],\"exclusions\":[],\"extraAttributes\":{},\"crossVersion\":{\"type\":\"Disabled\"}}":{"value":{"$fields":["path","startLine"],"path":"(sbt.Classpaths.jvmBaseSettings) Defaults.scala","startLine":2527},"type":"LinePosition"}}

==> scala/target/streams/_global/dependencyPositions/_global/streams/update_cache_2.12/output_dsp <==
{"{\"organization\":\"org.scala-lang\",\"name\":\"scala-library\",\"revision\":\"2.12.10\",\"isChanging\":false,\"isTransitive\":true,\"isForce\":false,\"explicitArtifacts\":[],\"inclusions\":[],\"exclusions\":[],\"extraAttributes\":{},\"crossVersion\":{\"type\":\"Disabled\"}}":{"value":{"$fields":["path","startLine"],"path":"(sbt.Classpaths.jvmBaseSettings) Defaults.scala","startLine":2527},"type":"LinePosition"}}

==> target/streams/$global/dependencyPositions/$global/streams/update_cache_2.12/output_dsp <==
{"{\"organization\":\"org.scala-lang\",\"name\":\"scala-library\",\"revision\":\"2.12.7\",\"isChanging\":false,\"isTransitive\":true,\"isForce\":false,\"explicitArtifacts\":[],\"inclusions\":[],\"exclusions\":[],\"extraAttributes\":{},\"crossVersion\":{\"type\":\"Disabled\"}}":{"value":{"$fields":["path","startLine"],"path":"(sbt.Classpaths.jvmBaseSettings) Defaults.scala","startLine":2207},"type":"LinePosition"}}

==> target/streams/compile/compile/$global/streams/out <==
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:2:16: object dsl is not a member of package spatial[0m
[0m[[0m[31merror[0m] [0m[0mimport spatial.dsl._[0m
[0m[[0m[31merror[0m] [0m[0m               ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:11:61: not found: type SpatialTest[0m
[0m[[0m[31merror[0m] [0m[0m@spatial abstract class cgo_conv(region: scala.Int) extends SpatialTest {[0m
[0m[[0m[31merror[0m] [0m[0m                                                            ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:11:2: not found: type spatial[0m
[0m[[0m[31merror[0m] [0m[0m@spatial abstract class cgo_conv(region: scala.Int) extends SpatialTest {[0m
[0m[[0m[31merror[0m] [0m[0m ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:12:12: not found: type FixPt[0m
[0m[[0m[31merror[0m] [0m[0m  type T = FixPt[TRUE,_16,_0][0m
[0m[[0m[31merror[0m] [0m[0m           ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:13:13: not found: type FixPt[0m
[0m[[0m[31merror[0m] [0m[0m  type T2 = FixPt[TRUE,_32,_0][0m
[0m[[0m[31merror[0m] [0m[0m            ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:14:16: not found: type FixPt[0m
[0m[[0m[31merror[0m] [0m[0m  type REALT = FixPt[TRUE,_4,_12][0m
[0m[[0m[31merror[0m] [0m[0m               ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:15:17: not found: type FixPt[0m
[0m[[0m[31merror[0m] [0m[0m  type REALT2 = FixPt[TRUE,_8,_24][0m
[0m[[0m[31merror[0m] [0m[0m                ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:28:22: Int(16) does not take parameters[0m
[0m[[0m[31merror[0m] [0m[0m    val loadPar = 16 (1 -> 16)[0m
[0m[[0m[31merror[0m] [0m[0m                     ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:29:23: Int(16) does not take parameters[0m
[0m[[0m[31merror[0m] [0m[0m    val storePar = 16 (1 -> 16)[0m
[0m[[0m[31merror[0m] [0m[0m                      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:31:22: not found: value ArgIn[0m
[0m[[0m[31merror[0m] [0m[0m    val INPUT_ROWS = ArgIn[Int][0m
[0m[[0m[31merror[0m] [0m[0m                     ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:32:22: not found: value ArgIn[0m
[0m[[0m[31merror[0m] [0m[0m    val INPUT_COLS = ArgIn[Int][0m
[0m[[0m[31merror[0m] [0m[0m                     ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:33:23: not found: value ArgIn[0m
[0m[[0m[31merror[0m] [0m[0m    val INPUT_CHANS = ArgIn[Int][0m
[0m[[0m[31merror[0m] [0m[0m                      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:34:24: not found: value ArgIn[0m
[0m[[0m[31merror[0m] [0m[0m    val OUTPUT_CHANS = ArgIn[Int][0m
[0m[[0m[31merror[0m] [0m[0m                       ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:36:18: not found: value ArgIn[0m
[0m[[0m[31merror[0m] [0m[0m    val STRIDE = ArgIn[Int] // Assume horiz and vert stride match[0m
[0m[[0m[31merror[0m] [0m[0m                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:41:33: Int takes no type parameters, expected: one[0m
[0m[[0m[31merror[0m] [0m[0m    val input_rows = args(0).to[Int][0m
[0m[[0m[31merror[0m] [0m[0m                                ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:42:33: Int takes no type parameters, expected: one[0m
[0m[[0m[31merror[0m] [0m[0m    val input_cols = args(1).to[Int][0m
[0m[[0m[31merror[0m] [0m[0m                                ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:43:34: Int takes no type parameters, expected: one[0m
[0m[[0m[31merror[0m] [0m[0m    val input_chans = args(2).to[Int][0m
[0m[[0m[31merror[0m] [0m[0m                                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:44:35: Int takes no type parameters, expected: one[0m
[0m[[0m[31merror[0m] [0m[0m    val output_chans = args(3).to[Int][0m
[0m[[0m[31merror[0m] [0m[0m                                  ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:45:29: Int takes no type parameters, expected: one[0m
[0m[[0m[31merror[0m] [0m[0m    val stride = args(4).to[Int][0m
[0m[[0m[31merror[0m] [0m[0m                            ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:46:33: not found: type Bit[0m
[0m[[0m[31merror[0m] [0m[0m    val print_data = args(5).to[Bit][0m
[0m[[0m[31merror[0m] [0m[0m                                ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:48:43: value r is not a member of StringContext[0m
[0m[[0m[31merror[0m] [0m[0m    if (P1 > 1) assert(output_chans > 16, r"Need at least 1 burst (oc=16) if P1 = $P1")[0m
[0m[[0m[31merror[0m] [0m[0m                                          ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:51:5: not found: value setArg[0m
[0m[[0m[31merror[0m] [0m[0m    setArg(INPUT_ROWS, input_rows)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:52:5: not found: value setArg[0m
[0m[[0m[31merror[0m] [0m[0m    setArg(INPUT_COLS, input_cols)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:53:5: not found: value setArg[0m
[0m[[0m[31merror[0m] [0m[0m    setArg(INPUT_CHANS, input_chans)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:54:5: not found: value setArg[0m
[0m[[0m[31merror[0m] [0m[0m    setArg(OUTPUT_CHANS, output_chans)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:55:5: not found: value setArg[0m
[0m[[0m[31merror[0m] [0m[0m    setArg(STRIDE, stride)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:63:22: not found: value DRAM[0m
[0m[[0m[31merror[0m] [0m[0m    val INPUT_DATA = DRAM[T](INPUT_COLS, INPUT_ROWS, INPUT_CHANS)[0m
[0m[[0m[31merror[0m] [0m[0m                     ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:64:23: not found: value DRAM[0m
[0m[[0m[31merror[0m] [0m[0m    val OUTPUT_DATA = DRAM[T]((INPUT_COLS-(KERNEL_COLS-STRIDE))/STRIDE, (INPUT_ROWS-(KERNEL_ROWS-STRIDE))/STRIDE, OUTPUT_CHANS)[0m
[0m[[0m[31merror[0m] [0m[0m                      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:65:23: not found: value DRAM[0m
[0m[[0m[31merror[0m] [0m[0m    val KERNEL_DATA = DRAM[T](OUTPUT_CHANS, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS)[0m
[0m[[0m[31merror[0m] [0m[0m                      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:66:23: not found: value DRAM[0m
[0m[[0m[31merror[0m] [0m[0m    val BIAS_DATA =   DRAM[T](OUTPUT_CHANS)[0m
[0m[[0m[31merror[0m] [0m[0m                      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:71:37: value :: is not a member of Int[0m
[0m[[0m[31merror[0m] [0m[0m    val kernel = (0::OUTPUT_CHANS, 0::KERNEL_COLS, 0::KERNEL_ROWS, 0::INPUT_CHANS) {(i,j,k,l) => if (random[Int](10) > 7) 64.to[T] else 0.to[T]}[0m
[0m[[0m[31merror[0m] [0m[0m                                    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:71:53: value :: is not a member of Int[0m
[0m[[0m[31merror[0m] [0m[0m    val kernel = (0::OUTPUT_CHANS, 0::KERNEL_COLS, 0::KERNEL_ROWS, 0::INPUT_CHANS) {(i,j,k,l) => if (random[Int](10) > 7) 64.to[T] else 0.to[T]}[0m
[0m[[0m[31merror[0m] [0m[0m                                                    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:71:102: not found: value random[0m
[0m[[0m[31merror[0m] [0m[0m    val kernel = (0::OUTPUT_CHANS, 0::KERNEL_COLS, 0::KERNEL_ROWS, 0::INPUT_CHANS) {(i,j,k,l) => if (random[Int](10) > 7) 64.to[T] else 0.to[T]}[0m
[0m[[0m[31merror[0m] [0m[0m                                                                                                     ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:71:126: overloaded method value to with alternatives:[0m
[0m[[0m[31merror[0m] [0m[0m  (end: Int,step: Int)scala.collection.immutable.Range.Inclusive <and>[0m
[0m[[0m[31merror[0m] [0m[0m  (end: Int)scala.collection.immutable.Range.Inclusive[0m
[0m[[0m[31merror[0m] [0m[0m does not take type parameters[0m
[0m[[0m[31merror[0m] [0m[0m    val kernel = (0::OUTPUT_CHANS, 0::KERNEL_COLS, 0::KERNEL_ROWS, 0::INPUT_CHANS) {(i,j,k,l) => if (random[Int](10) > 7) 64.to[T] else 0.to[T]}[0m
[0m[[0m[31merror[0m] [0m[0m                                                                                                                             ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:71:139: overloaded method value to with alternatives:[0m
[0m[[0m[31merror[0m] [0m[0m  (end: Int,step: Int)scala.collection.immutable.Range.Inclusive <and>[0m
[0m[[0m[31merror[0m] [0m[0m  (end: Int)scala.collection.immutable.Range.Inclusive[0m
[0m[[0m[31merror[0m] [0m[0m does not take type parameters[0m
[0m[[0m[31merror[0m] [0m[0m    val kernel = (0::OUTPUT_CHANS, 0::KERNEL_COLS, 0::KERNEL_ROWS, 0::INPUT_CHANS) {(i,j,k,l) => if (random[Int](10) > 7) 64.to[T] else 0.to[T]}[0m
[0m[[0m[31merror[0m] [0m[0m                                                                                                                                          ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:74:5: not found: value printTensor3[0m
[0m[[0m[31merror[0m] [0m[0m    printTensor3(input, "Input")[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:75:5: not found: value printTensor4[0m
[0m[[0m[31merror[0m] [0m[0m    printTensor4(kernel, "Kernel")[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:76:5: not found: value printArray[0m
[0m[[0m[31merror[0m] [0m[0m    printArray(bias, "Bias")[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:79:5: not found: value setMem[0m
[0m[[0m[31merror[0m] [0m[0m    setMem(INPUT_DATA, input)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:80:5: not found: value setMem[0m
[0m[[0m[31merror[0m] [0m[0m    setMem(OUTPUT_DATA, output)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:81:5: not found: value setMem[0m
[0m[[0m[31merror[0m] [0m[0m    setMem(KERNEL_DATA, kernel)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:82:5: not found: value setMem[0m
[0m[[0m[31merror[0m] [0m[0m    setMem(BIAS_DATA, bias)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:87:17: not found: value ArgOut[0m
[0m[[0m[31merror[0m] [0m[0m    val probe = ArgOut[T2][0m
[0m[[0m[31merror[0m] [0m[0m                ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:88:5: not found: value Accel[0m
[0m[[0m[31merror[0m] [0m[0m    Accel{[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:90:26: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        if (region == 0) SRAM[T](OUTPUT_CHANS_MAX, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS_MAX).effort(0).hierarchical.nBest.alphaBest.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                         ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:91:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 1) SRAM[T](OUTPUT_CHANS_MAX, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS_MAX).effort(0).hierarchical.nPow2.alphaPow2.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:92:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 2) SRAM[T](OUTPUT_CHANS_MAX, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS_MAX).effort(0).flat.nBest.alphaBest.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:93:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 3) SRAM[T](OUTPUT_CHANS_MAX, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS_MAX).effort(0).flat.nPow2.alphaPow2.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:94:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 4) SRAM[T](OUTPUT_CHANS_MAX, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS_MAX).effort(0).hierarchical.nBest.alphaBest.onlyblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:95:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 5) SRAM[T](OUTPUT_CHANS_MAX, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS_MAX).effort(0).hierarchical.nBest.alphaBest.noblockcyclic.axesfission(List(List(0)))[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:96:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 6) SRAM[T](OUTPUT_CHANS_MAX, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS_MAX).effort(0).flat.nBest.alphaBest.noblockcyclic.axesfission(List(List(0)))[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:97:14: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else SRAM[T](OUTPUT_CHANS_MAX, KERNEL_COLS, KERNEL_ROWS, INPUT_CHANS_MAX).effort(0).hierarchical[0m
[0m[[0m[31merror[0m] [0m[0m             ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:99:17: not found: value Reg[0m
[0m[[0m[31merror[0m] [0m[0m      val reg = Reg[T2](0).conflictable[0m
[0m[[0m[31merror[0m] [0m[0m                ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:102:7: not found: value Foreach[0m
[0m[[0m[31merror[0m] [0m[0m      Foreach(rowspan par P1){ R =>[0m
[0m[[0m[31merror[0m] [0m[0m      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:104:9: not found: value Foreach[0m
[0m[[0m[31merror[0m] [0m[0m        Foreach(colspan par P2){ C =>[0m
[0m[[0m[31merror[0m] [0m[0m        ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:106:11: not found: value Foreach[0m
[0m[[0m[31merror[0m] [0m[0m          Foreach(INPUT_CHANS by 1 par P3){ ic =>[0m
[0m[[0m[31merror[0m] [0m[0m          ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:107:13: not found: value Foreach[0m
[0m[[0m[31merror[0m] [0m[0m            Foreach(OUTPUT_CHANS by 1 par P4){ oc =>[0m
[0m[[0m[31merror[0m] [0m[0m            ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:111:50: missing parameter type for expanded function ((x$15: <error>, x$16) => x$15.$plus(x$16))[0m
[0m[[0m[31merror[0m] [0m[0m              val accum = filter_elements.reduce{_+_}[0m
[0m[[0m[31merror[0m] [0m[0m                                                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:111:52: missing parameter type for expanded function ((x$15: <error>, x$16: <error>) => x$15.$plus(x$16))[0m
[0m[[0m[31merror[0m] [0m[0m              val accum = filter_elements.reduce{_+_}[0m
[0m[[0m[31merror[0m] [0m[0m                                                   ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:116:11: not found: value Foreach[0m
[0m[[0m[31merror[0m] [0m[0m          Foreach(OUTPUT_CHANS by 1 par P6){i =>[0m
[0m[[0m[31merror[0m] [0m[0m          ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:119:23: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m          val dummy = SRAM[T](OUTPUT_CHANS_MAX)[0m
[0m[[0m[31merror[0m] [0m[0m                      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:127:12: not found: value getArg[0m
[0m[[0m[31merror[0m] [0m[0m    assert(getArg(probe).to[Int] == 5)[0m
[0m[[0m[31merror[0m] [0m[0m           ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:142:60: not found: type SpatialTest[0m
[0m[[0m[31merror[0m] [0m[0m@spatial abstract class cgo_fft(region: scala.Int) extends SpatialTest {[0m
[0m[[0m[31merror[0m] [0m[0m                                                           ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:142:2: not found: type spatial[0m
[0m[[0m[31merror[0m] [0m[0m@spatial abstract class cgo_fft(region: scala.Int) extends SpatialTest {[0m
[0m[[0m[31merror[0m] [0m[0m ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:148:12: not found: type FixPt[0m
[0m[[0m[31merror[0m] [0m[0m  type T = FixPt[TRUE,_16,_16][0m
[0m[[0m[31merror[0m] [0m[0m           ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:155:44: overloaded method value to with alternatives:[0m
[0m[[0m[31merror[0m] [0m[0m  (end: Double,step: Double)scala.collection.immutable.NumericRange.Inclusive[Double] <and>[0m
[0m[[0m[31merror[0m] [0m[0m  (end: Double)Range.Partial[Double,scala.collection.immutable.NumericRange[Double]][0m
[0m[[0m[31merror[0m] [0m[0m does not take type parameters[0m
[0m[[0m[31merror[0m] [0m[0m    val M_SQRT1_2 = 0.70710678118654752440.to[T][0m
[0m[[0m[31merror[0m] [0m[0m                                           ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:156:34: overloaded method value to with alternatives:[0m
[0m[[0m[31merror[0m] [0m[0m  (end: Double,step: Double)scala.collection.immutable.NumericRange.Inclusive[Double] <and>[0m
[0m[[0m[31merror[0m] [0m[0m  (end: Double)Range.Partial[Double,scala.collection.immutable.NumericRange[Double]][0m
[0m[[0m[31merror[0m] [0m[0m does not take type parameters[0m
[0m[[0m[31merror[0m] [0m[0m    val TWOPI = 6.28318530717959.to[T][0m
[0m[[0m[31merror[0m] [0m[0m                                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:158:18: not found: value loadCSV1D[0m
[0m[[0m[31merror[0m] [0m[0m    val data_x = loadCSV1D[T](s"$DATA/fft/fft_transpose_x.csv", "\n").reshape(8,stride)[0m
[0m[[0m[31merror[0m] [0m[0m                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:158:34: not found: value DATA[0m
[0m[[0m[31merror[0m] [0m[0m    val data_x = loadCSV1D[T](s"$DATA/fft/fft_transpose_x.csv", "\n").reshape(8,stride)[0m
[0m[[0m[31merror[0m] [0m[0m                                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:159:18: not found: value loadCSV1D[0m
[0m[[0m[31merror[0m] [0m[0m    val data_y = loadCSV1D[T](s"$DATA/fft/fft_transpose_y.csv", "\n").reshape(8,stride)[0m
[0m[[0m[31merror[0m] [0m[0m                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:159:34: not found: value DATA[0m
[0m[[0m[31merror[0m] [0m[0m    val data_y = loadCSV1D[T](s"$DATA/fft/fft_transpose_y.csv", "\n").reshape(8,stride)[0m
[0m[[0m[31merror[0m] [0m[0m                                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:161:23: not found: value DRAM[0m
[0m[[0m[31merror[0m] [0m[0m    val work_x_dram = DRAM[T](8,stride)[0m
[0m[[0m[31merror[0m] [0m[0m                      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:162:23: not found: value DRAM[0m
[0m[[0m[31merror[0m] [0m[0m    val work_y_dram = DRAM[T](8,stride)[0m
[0m[[0m[31merror[0m] [0m[0m                      ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:163:25: not found: value DRAM[0m
[0m[[0m[31merror[0m] [0m[0m    val result_x_dram = DRAM[T](8,stride)[0m
[0m[[0m[31merror[0m] [0m[0m                        ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:164:25: not found: value DRAM[0m
[0m[[0m[31merror[0m] [0m[0m    val result_y_dram = DRAM[T](8,stride)[0m
[0m[[0m[31merror[0m] [0m[0m                        ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:166:17: not found: value ArgOut[0m
[0m[[0m[31merror[0m] [0m[0m    val probe = ArgOut[T][0m
[0m[[0m[31merror[0m] [0m[0m                ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:167:5: not found: value setMem[0m
[0m[[0m[31merror[0m] [0m[0m    setMem(work_x_dram, data_x)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:168:5: not found: value setMem[0m
[0m[[0m[31merror[0m] [0m[0m    setMem(work_y_dram, data_y)[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:170:5: not found: value Accel[0m
[0m[[0m[31merror[0m] [0m[0m    Accel{[0m
[0m[[0m[31merror[0m] [0m[0m    ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:172:26: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        if (region == 0) SRAM[T](8,stride).effort(0).hierarchical.nBest.alphaBest.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                         ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:173:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 1) SRAM[T](8,stride).effort(0).hierarchical.nPow2.alphaPow2.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:174:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 2) SRAM[T](8,stride).effort(0).flat.nBest.alphaBest.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:175:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 3) SRAM[T](8,stride).effort(0).flat.nPow2.alphaPow2.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:176:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 4) SRAM[T](8,stride).effort(0).hierarchical.nBest.alphaBest.onlyblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:177:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 5) SRAM[T](8,stride).effort(0).hierarchical.nBest.alphaBest.noblockcyclic.axesfission(List(List(0)))[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:178:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 6) SRAM[T](8,stride).effort(0).flat.nBest.alphaBest.noblockcyclic.axesfission(List(List(0)))[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:179:14: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else SRAM[T](8,stride).effort(0).hierarchical[0m
[0m[[0m[31merror[0m] [0m[0m             ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:181:26: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        if (region == 0) SRAM[T](8,stride).effort(0).hierarchical.nBest.alphaBest.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                         ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:182:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 1) SRAM[T](8,stride).effort(0).hierarchical.nPow2.alphaPow2.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:183:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 2) SRAM[T](8,stride).effort(0).flat.nBest.alphaBest.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:184:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 3) SRAM[T](8,stride).effort(0).flat.nPow2.alphaPow2.noblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:185:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 4) SRAM[T](8,stride).effort(0).hierarchical.nBest.alphaBest.onlyblockcyclic.nofission[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:186:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 5) SRAM[T](8,stride).effort(0).hierarchical.nBest.alphaBest.noblockcyclic.axesfission(List(List(0)))[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:187:31: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else if (region == 6) SRAM[T](8,stride).effort(0).flat.nBest.alphaBest.noblockcyclic.axesfission(List(List(0)))[0m
[0m[[0m[31merror[0m] [0m[0m                              ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:188:14: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m        else SRAM[T](8,stride).effort(0).hierarchical[0m
[0m[[0m[31merror[0m] [0m[0m             ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:189:18: not found: value SRAM[0m
[0m[[0m[31merror[0m] [0m[0m      val smem = SRAM[T](8*8*9)[0m
[0m[[0m[31merror[0m] [0m[0m                 ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:194:26: not found: value LUT[0m
[0m[[0m[31merror[0m] [0m[0m      val reversed_LUT = LUT[Int](8)(0,4,2,6,1,5,3,7)[0m
[0m[[0m[31merror[0m] [0m[0m                         ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:196:26: not found: type I32[0m
[0m[[0m[31merror[0m] [0m[0m      def twiddles8(tid: I32, i: Int, N: Int): Unit = {[0m
[0m[[0m[31merror[0m] [0m[0m                         ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:197:9: not found: value Foreach[0m
[0m[[0m[31merror[0m] [0m[0m        Foreach(1 until 8 by 1) { j =>[0m
[0m[[0m[31merror[0m] [0m[0m        ^[0m
[0m[[0m[31merror[0m] [0m[0m/home/mattfel/pldi/docs/pldi.scala:202:29: not found: value mux[0m
[0m[[0m[31merror[0m] [0m[0m          val phi_bounded = mux(beyond_left, phi_shifted + TWOPI.to[T]/2, mux(beyond_right, phi_shifted - TWOPI.to[T]/2, phi_shifted))[0m
[0m[[0m[31merror[0m] [0m[0m                            ^[0m
[0m[[0m[31merror[0m] [0m[0m622 errors found[0m


==> text/__latexindent_temp.tex <==
\section{Background}
\label{background}

\textit{Memory banking} is the process of partitioning a multidimensional array so that it can be implemented in hardware as a collection of physical BRAM resources and surrounding logic to index into them.
In this paper, we refer to the access pattern to an array in the program as the \textit{logical} access (i.e. \texttt{arr[2*i+3]}), and the circuits which connect to BRAMs as \textit{physical} accesses.

\subsection{Representing The Problem Using the Polyhedral Model}
The \textit{polyhedral model} \cite{memwithpoly} is a formalism for representing a program's iteration space, memory space, and access patterns in a compact way that a compiler can statically analyze.
We use it as a tool to solve the banking problem, and briefly summarize the important concepts used in prior work \cite{cong}.

\begin{definition}{A \textit{Polyhedron}}
	is a set of points in n-dimensional space that satisfy a set of linear inequalities.  Namely, the set of points $P = \{\vec{x} \in \mathbb{Q}^n | A\cdot\vec{x}\leq \vec{b}\}$ where $\mathbb{Q}^n$ is an n-dimensional vector of rational numbers, A is a matrix where $A_{i,j}\in \mathbb{Q}$, and $\vec{b}\in \mathbb{Q}^n$.
\end{definition}
\begin{definition}{A \textit{Polytope}}
	is a bounded polyhedron, e.g. one that contains a finite amount of integer points.
\end{definition}
\begin{definition}{A \textit{Parallelotope}} is a polytope where every pair of opposite facets are congruent and parallel, i.e. the n-dimensional generalization of a parallelogram (2D) or parallelepiped (3D).
\end{definition}
\begin{definition}{The \textit{iterator space}}
	is a polytope defined by the iterators, $\vec{i}$, of a loop nest. 
	%We require that all iterators start at 0 and have a stride of 1. 
	%In the case of an iterator, $k$, in the form \texttt{for (k = B -> S -> E par P)}, we express it in the form $k_\ell = i_\ell*S*P + B + \ell*S$  $\forall i_\ell \in \{0,..,\ceil{\frac{E-\left(B + \ell \cdot S\right)}{S\cdot P}}\}, \ell \in \{0,..,P-1\}$.
	%We refer to $\ell$ as the ``lane."
\end{definition}
\begin{definition}{An \textit{array}}
	is an n-dimensional on-chip memory whose addresses represent a polytope
\end{definition}
\begin{definition}{An \textit{access pattern} for access $a$}
	is an expression representing the mapping from the iterator space to an n-dimensional reference to the array polytope.
\end{definition}
\begin{definition}{An \textit{access group}}
	is a collection of access patterns which can be active during the same cycle at runtime.
\end{definition}


\subsection{Partitioning Methods}

\begin{figure}
	\centering
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=0.75\textwidth]{figs/hyperplane-eps-converted-to.pdf}
		\caption{}
		\label{fig:hyperplane}
	\end{subfigure}
	~
	\begin{subfigure}{0.23\textwidth}
		\centering
		\includegraphics[width=0.75\textwidth]{figs/lattice-eps-converted-to.pdf}
		\caption{}
		\label{fig:lattice}
	\end{subfigure}
	
	\caption{Example 4x4 array partitioned into 4 banks using (a) hyperplane and (b) lattice.  Color represents bank}
	\label{fig:hyperplanelattice}	
	\vskip-.1in
\end{figure}

There are two common methods for partitioning the memory: \textit{hyperplane partitioning} \cite{cong} and \textit{lattice partitioning} \cite{latticepartition}, sketched in Figure \ref{fig:hyperplanelattice}.
Under hyperplane partitioning, the array polytope is divided into parallel ``hyperplanes," where each hyperplane represents a bank.
Under lattice partitioning, the array is divided into a tessellation of congruent parallelotopes, where each position within the parallelotope is assigned to a unique bank.
While most common partitioning problems have both hyperplane and lattice solutions, there are certain patterns where only one can provide a solution.
For example, hyperplane partitioning can solve problems that require a \textit{block-cyclic} pattern of banks, while lattice partitioning can solve problems with concurrent accesses that do not lie within a rectangular parallelotope

In this paper, we introduce a system based on hyperplane partitioning with an extension that captures a subset of lattice partitioning solutions, namely those composed of orthogonal parallelotopes.  
These are referred to as ``multidimensional" hyperplane geometries and are discussed in \ref{projections}.

Table \ref{table:params} concisely summarizes all of the quantities involved in our banking system.
\textbf{Input parameters} are provided by the SDH framework and represent the access pattern the programmer specified in the code.
\textbf{Solve parameters} are computed by our banking system.
Our system internally computes a collection of these but only returns the optimal set.
\textbf{Metrics} which are helpful quantities for understanding how the partitioning scheme will map to hardware.

\begin{table}
	\begin{tabular}{Lll}
		\toprule
		\textbf{Type} & \textbf{Name} & \textbf{Description} \\
		\midrule
		\multirow{5}{1cm}{Input} & $\vec{D}$ & Dimensions of memory, $|\vec{D}|=n$ \\
		& $\vec{a}$ & Logical accesses, grouped by concurrency \\
		& $\vec{i}$ & iterators in the scope of an access \\
		& $\vec{x}$ & Memory address reference for an access, $|\vec{x}| = n$      \\
		& $\textit{k}$ & Number of ports on underlying BRAM \\
		\midrule
		\multirow{4}{1cm}{Solve} & $\vec{N}$ & Number of banks, $|\vec{N}|\in\{1,n\}$ \\
		& $\vec{B}$ & Blocking factor, $|\vec{B}| = |\vec{N}|$      \\
		& $\vec{\alpha}$ & Partition vector, $|\vec{\alpha}|=n$    \\
		& $\vec{P}$ & Partition parallelotope,  $|\vec{P}|=n$      \\		\midrule
		\multirow{3}{1cm}{Metrics} & $FO_a$ & \# of banks an access touches (Fan-Out), \\
		& & $FO_a\leq\prod \vec{N}$ \\
		& $FI_b$ & \# of accesses a bank feeds (Fan-In),\\ 
		& & $\sum{FI_b} = \sum{FO_a}$ \\
		& $\vec{\delta}$ & Per-dimension padding\\
		\bottomrule
	\end{tabular}
	\caption{Partitioning parameters and definitions.}
	\label{table:params}
	%	\vskip-0.3in
\end{table}


Equations \ref{eq:BA} and \ref{eq:BO} show how the solve parameters are used to compute a \textbf{bank address ($BA$)} and \textbf{offset ($BO$)}. 
We refer to these collectively as the ``bank resolution" equations.

%\noindent\begin{minipage}[t][][b]{0.45\linewidth}
%$\displaystyle
%BA = \floor{\frac{\vec{x}\cdot\vec{\alpha}}{B}} \bmod{N}
%$
%\begin{equation}\label{eq:BA}\end{equation}
%\end{minipage}\hspace{5px}
%\begin{minipage}{0.52\linewidth}
%$\displaystyle R = \sum_{i=0}^n\left(\floor{\frac{\vec{x}_i}{\vec{P}_i}} \cdot\prod_{j=i+1}^n\ceil{\frac{\vec{D_j}}{\vec{P_j}}}\right)$ \\
%%$\displaystyle C = \sum_{i=0}^{n}{\left(\vec{x_i}\cdot\vec{\alpha_i}\right) \bmod B}$ \\
%$\displaystyle BO = R * B + C$
%\begin{equation}\label{eq:BO}\end{equation}
%
%\end{minipage}

\begin{equation}
\label{eq:BA}
BA = \floor{\frac{\vec{x}\cdot\vec{\alpha}}{B}} \bmod{N}
\end{equation}
\begin{equation}
\label{eq:BO}
BO = \left[B \cdot \sum_{i=0}^n\left(\floor{\frac{\vec{x}_i}{\vec{P}_i}} \cdot\prod_{j=i+1}^n\ceil{\frac{\vec{D_j}}{\vec{P_j}}}\right)\right] + \left(\vec{x}\cdot\vec{\alpha}  \bmod B\right)
\end{equation}



The equation for $BA$ divides the array polytope into parallel hyperplanes, and we therefore refer to $\vec{\alpha}$, $N$, and $B$ as representing a ``hyperplane geometry."
The parameter $\vec{P}$ is only used to compute a physical offset, and a hyperplane geometry may have many valid choices for $\vec{P}$.
It is related to the periodicity of Equation \ref{eq:BA} and represents a region in the array such that each $BA$ appears at least once and no more than $B$ times.

\begin{definition}{A \textit{conflict polytope} is the polytope generated by applying Equation \ref{eq:BA} to the delta between the address patterns of two different accesses ($BA(\vec{x}_{a_1}-\vec{x}_{a_2})$)}
\end{definition}
\begin{definition}{A hyperplane geometry is deemed \textit{valid} for a $k$-ported memory}
	if no set of $k$ accesses contain more than $k-1$ pairs of non-empty conflict polytopes.
\end{definition}

These definitions allow our system to handle addresses with non-affine components using quantifier-free Presburger arithmetic \cite{presberder}.  
Namely, any function call without side-effects (including indirection arrays) that is used in an address expression (i.e. \texttt{f($i_0$)} in \texttt{arr[f($i_0$) + $i_1$]}) can be represented an uninterpreted function symbol.  
This means that even though the compiler cannot analyze $BA($\texttt{f($i_0$) + $i_1$}$)$, it \textit{can} analyze any conflict polytope it generates against another access containing the same function symbol.

Finally, $FO_a$ and $FI_b$ describe the fan-out of accesses and fan-in of banks, respectively. 
They describe the size of the crossbars required to arbitrate between accesses and banks.
If $\vec{P}_i$ does not evenly divide $\vec{D}_i$, then the banking equations result in mathematically ``inaccessible" elements that require the compiler to pad the array with $\vec{\delta}$.
When $B>1$, there may be more inaccessible elements due to unequal representation of each bank within a $\vec{P}$ region.

\subsection{Consequences of Parameters}
\label{consequences}
The values of $\vec{N}$, $\vec{B}$, $\vec{\alpha}$, and $\vec{P}$ have implications on the overall FPGA resource utilization and latency of the circuit, since they impact the bank resolution logic, crossbar sizes, and bank volumes which must all map to quantized resources on the FPGA.

Consider the snippet in Figure \ref{fig:toy} with access patterns $6\cdot i + 1$, $6\cdot i + 2$, $6\cdot i + 4$, and $6\cdot i + 5$ (we substitute $k$ for unit-step iterator $i$).
Figure \ref{fig:options} shows three potential ways this problem can be solved.

\begin{figure}
	\begin{subfigure}{0.27\textwidth}
		\centering
		\begin{tabular}{p{0.2\linewidth}}
			\toprule
			{\begin{lstlisting}[language=Spatial,linewidth=0.98\columnwidth, mathescape=true]
				for (k = 0->3->M par 2) { 
				.. = arr[k+1] + arr[k+2];
				}
				\end{lstlisting}}\\
			\bottomrule
		\end{tabular}
		\caption{}
		\label{fig:toy}
	\end{subfigure}
	~
	\begin{subfigure}{0.2\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figs/options-eps-converted-to.pdf}
		\caption{}
		\label{fig:options}	
	\end{subfigure}
	\caption{(a) Sample access pattern with iterator $k$ start=0, step=3, stop=M, and parallelization=2. (b) Three valid banking schemes for \texttt{arr} with $BA$ values shown.}
	\label{fig:sample}	
	\vskip-.1in
\end{figure}

Option 1 uses 5 banks and full crossbars for each access ($FO_a$ = 5).
Option 2 appears better since it uses only 4 banks and $FO_a$ = 1, but requires a costly divide-by-3 and a multiply-by-2 operation.  
Option 3 uses 6 banks but achieves $FO_a$ = 1 while also eliminating B and $\alpha$ arithmetic.
Depending on the size of the array and the target FPGA, the volume of one ``bank" may spill into 2 BRAMs, so solutions with smaller $N$ may consume \textit{more} BRAMs.

The key point is that there are always many solutions to a banking problem and it is difficult to predict which one is the best.
Additionally, the definition of ``best" may change depending on which resource is scarcest for a given application.




\subsection{Concepts in Hierarchically-Nested State Machine Programming}
\label{progmodel}
A programming model based on parallel patterns \cite{parallelpatterns} is a good starting point for exposing a high level of abstraction without losing handles on performance \cite {spatial}.
For this reason, we chose to use Spatial as the host compiler for our banking system since it an open source, extensible language that can express massive design spaces, an explicit memory hierarchy, and multi-level parallelism.	

Our system targets programs composed as a set of hierarchically nested state machines, or \textit{controllers}.
A \textit{controller} is expressed as traditional software loop, and is represented in the IR as a multi-level counter chain that feeds iterator values to a basic block. 
A \textit{multi-level counter chain} is a counter that spans a multi-dimensional iteration space whose bounds do not need to be compile-time static.

\subsubsection{Controller Level} 
The contents of a controller's basic block define it's \textit{level}:

\begin{itemize}
	\item \textbf{Inner controllers} only contain dataflow graphs
	\item \textbf{Outer controllers} only contain other controllers
\end{itemize}

An outer controller and the controllers in its basic block define a \textit{parent-child} relationship in the controller hierarchy.
An outer controller's \textit{width} is the number of children it contains.
A controller's \textit{sub-tree} is the set of controllers found by following its children recursively.
A node's \textit{ancestors} is a list of every controller in the hierarchy that encloses it.
The \textit{least common ancestor} (LCA) of two nodes is the most deeply-nested controller which they both share.

\subsubsection{Controller Schedule}
\label{schedules}
"Scheduling" refers to how nodes in a controller's basic block execute relative to each other, but has different meanings for inner and outer controllers.

For outer controllers, there are five schedules describing how the children execute in hardware:
\begin{itemize}
	\item \texttt{Sequential} - Child controllers execute one at a time with no overlap.
	\item \texttt{Pipelined} - Child controllers execute in pipelined  (i.e. overlapping) fashion.
	\item \texttt{Fork-Join} - Child controllers execute simultaneously and independently of each other.  
	\item \texttt{Fork} - One child controller executes per iteration, based on a set of \texttt{if/then/else} conditions.
	\item \texttt{Streaming} - Child controllers execute as long as their input data is available. 
\end{itemize}

For inner controllers, the schedule refers to the mapping from each node in the pipelined dataflow graph to the cycle it will execute.
Scheduling nodes to execute during different cycles allows the design to safely run at a higher clock rate.
Their runtime is entirely defined by their \textit{latency}, which is the cycle at which its latest node is scheduled, and its \textit{initiation interval}, which is the number of cycles the controller must wait before it can increment the multi-level counter and issue another iteration.
The hardware-complexity of the datapath determines the latency, and the loop-carry dependencies determine the initiation interval.


\subsubsection{Controller Parallelization}
\label{pommop}
Parallelization is one of the ways that programs mapped to FPGA can improve performance.
Specifically, parallelizing a loop by $P$ means that $P$ consecutive iterations of the loop will be executed simultaneously.
To a first order approximation, this means that parallelization results in a factor of $P$ performance improvement by using $P$-times as many resources compared to the un-parallelized loop.

In reality, this typically improves performance by less than $P$ and increases resource utilization by more than $P$.
This is because initiation interval and latency may change with parallelization.
We must distinguish between parallelization of inner and outer controllers separately to understand why.

We walk through the example snippet in Figure \ref{fig:parexample} to demonstrate this.

Parallelization applied to an inner controller results in \textit{vectorization} of the datapath.  
Figure \ref{fig:innervec} shows how this is done for loop \texttt{k} with \texttt{IP} = 2.

Parallelization applied to an outer controller results in \textit{unrolling}.
Each child controller is cloned in whole and added to the hierarchy.
This is shown in Figure \ref{fig:pommop} as the "Pre-Unrolled" tree structure is transformed into the "Intermediate" structure for \texttt{OP} = 2.
The compiler must then inject \texttt{Fork-Join} controllers to this intermediate structure to achieve the parallelism specified in the program.
There are two strategies that the compiler may employ to capture this level of parallelism, shown in the "Post-Unrolled" trees in Figure \ref{fig:pommop}:
\begin{itemize}
	\item \textit{ForkJoin-of-Pipelines unrolling} is when the \texttt{Fork-Join} controllers are injected \textit{between} the outer controller and child stages such that all lanes of each child are synchronized (i.e. always begin their execution simultaneously). This guarantees that child \texttt{c} will not begin executing iteration \texttt{i+P} until iterations \texttt{i/P*P} to \textit{(i/P*P) + P - 1} are completed, for any child and iteration of the parent controller.
	\item \textit{Pipeline-of-ForkJoins unrolling} is when each lane of the original outer is separated into its own controller that is structurally identical to the pre-unrolled loop. A single \texttt{Fork-Join} controller is injected \textit{above} the outer controllers, such that all lanes begin executing simultaneously.  This guarantees that child \texttt{c} will not begin executing iteration \texttt{i+P} until iteration \texttt{i} is completed, for any child and iteration of the parent controller.  
	However, there is no guarantee about the relative ordering between iteration \texttt{i/P*P} and \texttt{i/P*P+K}, where \texttt{K \% P != 0}.
\end{itemize} 
\todo{SBS/LBS -> PoF/FoP in the figure}

For any node in the IR, its "unroll ID" (UID) is a list of integers describing which lane of each ancestor controller it belongs to.
The UID of a node is described as the "base UID" if all integers in the UID are 0.


\begin{figure}
	\centering
	\begin{tabular}{p{\linewidth}}
		\toprule
		{\begin{lstlisting}[language=Spatial,linewidth=0.98\columnwidth, mathescape=true]
			// Parent (Outer Ctrl)
			Foreach(N by 1 par OP){i =>  
			// Child 0
			Foreach(M by 1){j => /*...*/}
			// Child 1 (Inner Ctrl)
			Foreach(K by 1 par IP){k => 
			val t = i*3
			mem(k) = mux(k == 0, t + mem(k), t)
			}
			}
			\end{lstlisting}}\\
		\bottomrule
	\end{tabular}
	\vspace{-5pt}
	\caption{Example construction of an outer controller (Loop \texttt{i}) with parallelization (\texttt{OP}) and two child controllers (Loops \texttt{j} and \texttt{k}).  Loop \texttt{k} has parallelization factor \texttt{IP}.}
	\label{fig:parexample}
	
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.47\textwidth]{figs/vectorize-eps-converted-to.pdf}
	\caption{Dataflow path for the inner controller of loop \texttt{k} in Figure \ref{fig:parexample} before and after applying vectorization (IP=2).}
	\label{fig:innervec}
	
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.47\textwidth]{figs/pommop-eps-converted-to.pdf}
	\caption{Controller trees before and after unrolling loop i in Figure \ref{fig:parexample} (OP=2, IP=2) for stage-based and lane-based synchronization.}
	\label{fig:pommop}
	
\end{figure}


==> text/correction.tex <==
\section{Bank Offset Correction Calculation}
\label{correction}

As far as we are aware, prior papers outlining the implementation of the bank resolution equations (Equations 1 and 2)
%\ref{eq:BA} and \ref{eq:ofs}) 
do not explicitly provide a formula for addressing intra-bank offset when B > 1.
When B = 1, the neighborhood vector, $\vec{P}$ scopes out a hypercube where each bank is represented once.  
When B > 1, $\vec{P}$ must be selected such that each bank appears \textit{at most} B times.

The intuition behind the intra-bank correction, $C$, in Equation 2
%~\ref{eq:ofs} 
comes from the idea of periodicity per-dimension in the bank address equation (Equation 1)
%\ref{eq:BA}).
Equation \ref{eq:phi} shows how to use the least common multiple of certain parameters to compute this periodicity, $\vec{\Phi}$.  

\begin{equation}
\label{eq:phi}
	\vec{\Phi_i} = \frac{lcm(\vec{\alpha_i},NB)}{\vec{\alpha_i}}
\end{equation}

Because intra-bank offset (Equation 2)
%\ref{eq:ofs}) 
depends on floor division of an address by $B$ under modulo $N$, we are guaranteed that no neighborhood can contain more than $B$ unique instances of a single bank because of this periodicity.
Computing the dot product $\vec{x}\cdot\vec{\alpha}$ and applying modulo $B$ to this quantity distinguishes multiple instances of the same bank in a neighborhood uniquely.
In cases where $\alpha_i$ and $NB$ are not co-prime (i.e. $\Phi_i < NB$), then it is possible to substitute $B$ with $\ceil{\frac{\vec{\Phi_i}}{B}}$ in the intra-bank offset calculations.

Consider the simple example in Figure \ref{fig:correction} for N = 4, B = 2, $\alpha$ = 3, and P = $\Phi$ = 8.
The color of each cell represents its bank and the intra-bank offset is labeled with an integer over the cell.
The intra-bank correction is required so that no cells of the same bank have the same intra-bank offset.

\begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{figs/correction-eps-converted-to.pdf}
	\caption{Example showing how intra-bank offset correction properly labels an example where N=4, B = 2, $\alpha$ = 3 and P = $\Phi$ = lcm(3,4*2)/3 = 8. }
	\label{fig:correction}
	
\end{figure}




==> text/model_param.tex <==
\section{Model Learning Curves and Parameters}
\label{model_param}
Figures \ref{fig:learning_curves_ffs}, \ref{fig:learning_curves_ramb18}, and \ref{fig:learning_curves_ramb32}, as well as Table \ref{tab:eval} show the learning curves and parameters for the ML model.

\newcommand{\mmrow}[1]{\multirow{5}{*}{#1}}
\newcommand{\mmmrow}[1]{\multirow{4}{*}{#1}}

\begin{table*}[ht]
  \centering
    \begin{tabular}{@{} lllll *{2}{l} @{}}
    \toprule
      % \mrow{\textbf{Model}} & \multirow{2}{*}{\textbf{Model architecture}} & \multicolumn{2}{c@{}}{\textbf{Training parameters}}  & \multicolumn{2}{c@{}}{\textbf{Regularization parameters}}\\
      \textbf{Model} & \multicolumn{2}{c@{}}{\textbf{Model architecture}} & \multicolumn{2}{c@{}}{\textbf{Training parameters}}  & \multicolumn{2}{c@{}}{\textbf{Regularization parameters}} \\
      \midrule
        \mmrow{Ours}  &\textbf{random state}              & 30    & \textbf{objective}       & mean-squared error & \textbf{subsample}              & 0.6   \\
                            &\textbf{number of estimators}      & 159   & \textbf{learning rate (lr)}   & 0.1                & \textbf{col sample by tree}  & 1     \\
                            &\textbf{max tree depth}            & 3     &                          &                    & \textbf{$\lambda$}              & 0.04  \\
                            &\textbf{min samples split}         & 10    &                          &                    & \textbf{$\alpha$}               & 3     \\
                            &                                   &       &                          &                    & \textbf{$\gamma$}               & 5     \\ \addlinespace
      \midrule
        \mmmrow{MLP} &\textbf{hidden states}             & [128, 32, 32, 16]     & \textbf{objective}              & mean-squared error & \textbf{$\alpha$}              &  0.07      \\
                     &\textbf{activation}                & \textit{relu}         & \textbf{learning rate (lr)}     & adaptive           &   &       \\
                     &                                   &                       & \textbf{initial lr}             & 0.0015             &                                 &       \\
                     &                                   &                       & \textbf{power\_t}               & 0.5                &                                 &          \\ \addlinespace
      \bottomrule
      \addlinespace
    \label{table:model_parameters}
    \end{tabular}

  \caption{Final parameters of the evaluated models.}\label{tab:eval}
\end{table*}

\begin{figure*}[!tbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth, height=2in]{figs/ffs_mlp_learning_curve_70_5.pdf}
      \caption{The baseline model.}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth, height=2in]{figs/ffs_xgdb_learning_curve_75_34.pdf}
      \caption{The proposed pipeline.}
    \end{subfigure}
    \caption{Learning curves of the baseline model (left) and our proposed model pipeline when predicting FF utilization.}
    \label{fig:learning_curves_ffs}
\end{figure*}

\begin{figure*}[!tbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth, height=2in]{figs/ramb18_mlp_learning_curve_56_77.pdf}
      \caption{The baseline model.}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth, height=2in]{figs/ramb18_xgdb_learning_curve_72_57.pdf}
      \caption{The proposed pipeline.}
    \end{subfigure}
    \caption{Learning curves of the baseline model (left) and our proposed model pipeline when predicting RAMB18 utilization.
    The baseline model starts to overfit on the dataset despite of all the regularization introduced. 
    However, our pipeline still manages to achieve high performance without overfitting.}
    \label{fig:learning_curves_ramb18}
\end{figure*}

\begin{figure*}[!tbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth, height=2in]{figs/ramb32_mlp_learning_curve_73_35.pdf}
      \caption{The baseline model.}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth, height=2in]{figs/ramb32_xgdb_learning_curve_81_22.pdf}
      \caption{The proposed pipeline.}
    \end{subfigure}
    \caption{Learning curves of the baseline model (left) and our proposed model pipeline when predicting RAMB36 utilization.
    We observed that the FPGA PnR tool mapped small memory to RAMB36 less frequently.
    Hence, the training data for RAMB36 is much less than the other resource types.
    As a result, the standard deviations for both models are very high. }
    \label{fig:learning_curves_ramb32}
\end{figure*}


==> text/target/streams/_global/dependencyPositions/_global/streams/update_cache_2.12/output_dsp <==
{"{\"organization\":\"org.scala-lang\",\"name\":\"scala-library\",\"revision\":\"2.12.10\",\"isChanging\":false,\"isTransitive\":true,\"isForce\":false,\"explicitArtifacts\":[],\"inclusions\":[],\"exclusions\":[],\"extraAttributes\":{},\"crossVersion\":{\"type\":\"Disabled\"}}":{"value":{"$fields":["path","startLine"],"path":"(sbt.Classpaths.jvmBaseSettings) Defaults.scala","startLine":2523},"type":"LinePosition"}}
